Test-Time Optimization for Domain Adaptive Open Vocabulary Segmentation

We present Seg-TTO, a novel framework for zero-shot, open-vocabulary semantic segmentation (OVSS), designed to excel in specialized domain tasks. While current open-vocabulary approaches show impressive performance on standard segmentation benchmarks under zero-shot settings, they fall short of supervised counterparts on highly domain-specific datasets. We focus on segmentation-specific test-time optimization to address this gap. Segmentation requires an understanding of multiple concepts within a single image while retaining the locality and spatial structure of representations. We propose a novel self-supervised objective adhering to these requirements and use it to align the model parameters with input images at test time. In the textual modality, we learn multiple embeddings for each category to capture diverse concepts within an image, while in the visual modality, we calculate pixel-level losses followed by embedding aggregation operations specific to preserving spatial structure. Our resulting framework termed Seg-TTO is a plug-and-play module. We integrate Seg-TTO with three state-of-the-art OVSS approaches and evaluate across 22 challenging OVSS tasks covering a range of specialized domains. Our Seg-TTO demonstrates clear performance improvements (up to 27% mIoU increase on some datasets) establishing new state-of-the-art. Our code and models will be released publicly.

==> figures/ablate_crop_selection.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]
    {images/crop_selection.png}
    \caption{\todo{replace table 6}}
    \label{fig:ablate_crop_selection}
    % \vspace{-1.0em}
\end{figure}

==> figures/ablate_prompt_steps.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]
    {images/prompts_and_steps.png}
    \caption{\todo{replace table 7}}
    \label{fig:ablate_prompt_steps}
    % \vspace{-1.0em}
\end{figure}

==> figures/attribute_plot.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{images/attribute_plot.pdf}\hfill\\
    \vspace{-10pt}
    \caption{\textbf{Performance across different ratios of class name with prompts to attributes}} 
    \label{fig:attribute_plot}\vspace{-10pt}
\end{figure}

==> tables/ablate_crops.tex <==
% \begin{table}[t]
% \centering
% \small
% \def\arraystretch{1.2}  % height
% \setlength\tabcolsep{0.8em}  % width
% \scalebox{0.95}{
% \begin{tabular}{cc|c}
% \toprule
% Number of crops & Selected percentage    &   DZ  \\ \midrule 
% 64    &  0.1 & 34.4 \\ \rowcolor{Gray}
% 64     &  0.2 & 34.6 \\  
% 64     &  0.3 & 32.7 \\ 
% 64     &  1.0 & 32.7 \\
% 32     &  0.1 & 34.3 \\ 
% 32    &  0.2  & 34.4 \\ 
% 16    & 0.2   &  33.1    \\ \bottomrule
% \end{tabular}
% }
% % \vspace{-1.0em}
% \caption{
% \textbf{Results under prompt tuning crop selection}: We ablate how augmentations used and their confidence affects the final segmentation performance.
%  % 
% }
% \label{tbl:crop_selection}
% \vspace{-1em}
% \end{table}

% % 128   & 0.1  &  \textbf{34.9}  \\

==> tables/ablate_main.tex <==
\begin{table}[t]
\centering
\small
\def\arraystretch{1.2}  % height
\setlength\tabcolsep{0.8em}  % width
\scalebox{0.95}{
\begin{tabular}{l|cccccc}
\toprule
Method   &  VAG   & DAS   & STPT   & ZWF  & DZ & Dram   \\ \midrule
CAT-Seg-L & \xmark & \xmark & \xmark & 30.6 & 33.1 & 66.5 \\
Ours     & \cmark & \xmark & \xmark & 31.8 & 33.5 & 69.2 \\
Ours     & \cmark & \cmark & \xmark & 31.9 & 34.2 & 69.8\\ \rowcolor{Gray}
Ours     & \cmark & \cmark & \cmark & 32.3 & 34.6 & 70.2\\ \bottomrule
\end{tabular}
}
% \vspace{-1.0em}
\caption{
\textbf{Ablation on \modelname}: 
We ablate each component of our proposed \modelname to highlight individual contributions. DAS, VAG, and STPT denote Dynamic Augmentation Selection, Visual Attribute Generation, and Segmentation specific Test-time Prompt Tuning. We perform these ablations on three out-of-domain segmentation datasets from the MESS Benchmark \cite{MESS}, ZeroWaste-F (ZWF), Dark Zurich (DZ) and Dram. 
}
\label{tbl:main_ablation}
\vspace{-1em}
\end{table}

% Method   &  VAG   & DAS   & STPT   & ZWF  & DZ   \\ \midrule
% Baseline & \xmark & \xmark & \xmark & 30.6 & 33.1 \\
% Ours     & \cmark & \xmark & \xmark & 31.8 & 33.5 \\
% Ours     & \cmark & \cmark & \xmark & 31.9 & 34.2 \\ \rowcolor{Gray}
% Ours     & \cmark & \cmark & \cmark & 32.3 & 34.6 \\ \bottomrule

==> tables/ablate_prompts.tex <==
% \begin{table}[t]
% \centering
% \small
% \def\arraystretch{1.2}  % height
% \setlength\tabcolsep{0.8em}  % width
% \scalebox{0.95}{
% \begin{tabular}{c|c}
% \toprule
% Number of prompts    &   DZ \\ \midrule
% 1     &  32.8 \\ 
% 2     &  32.6  \\
% 3     &  34.3 \\ 
% 4     &  32.7 \\ \rowcolor{Gray}
% 5     &  34.6 \\   
% 10    &  32.5  \\ \bottomrule
% \end{tabular}
% }
% % \vspace{-1.0em}
% \caption{
% \textbf{Results under a different number of prompts tuned}: 
%  % 
% }
% \label{tbl:ablate_num_prompts}
% \vspace{-1em}
% \end{table}


% % Number of prompts    &   DZ & SUIM   \\ \midrule
% % 1     &  32.8 & 57.6\\ 
% % 2     &  32.6 & 57.3 \\
% % 3     &  34.3 & 57.7 \\ 
% % 4     &  32.7 & 57.8\\ \rowcolor{Gray}
% % 5     &  34.6 & 57.8\\   
% % 10    &  32.5  & \\ \bottomrule

==> tables/ablate_tpt_steps.tex <==
% \begin{table}[t]
% \centering
% \small
% \def\arraystretch{1.2}  % height
% \setlength\tabcolsep{0.8em}  % width
% \scalebox{0.95}{
% \begin{tabular}{c|cc}
% \toprule
% \multirow{2}{*}{} & \multicolumn{2}{c}{Dark Zurich (DZ)} \\
% \cline{2-3}
%    &   Prompt tuning steps & Number of prompts  \\ \midrule
% 1     &  34.49 & 32.8 \\
% 2     &  \textbf{34.58} & 32.6 \\  
% 3     &  34.56 & 34.3 \\ 
% 4     &  34.56 & 32.7 \\
% 5     &  34.51 & \textbf{34.6} \\
% 10 & 34.4 & 32.5 \\ \bottomrule
% \end{tabular}
% }
% % \vspace{-1.0em}
% \caption{
% \textbf{Selecting prompts and tuning steps}: We ablate how changing the number of prompt tuning steps and the number of prompts used for tuning affects the results.
% % 
% }
% \label{tbl:tpt_steps}
% \vspace{-1em}
% \end{table}

% Prompt tuning steps   &   DZ  \\ \midrule
% 1     &  34.49 \\ \rowcolor{Gray}
% 2     &  34.58 \\  
% 3     &  34.56 \\ 
% 4     &  34.56 \\
% 5     &  34.51 \\
% 10 & 34.4 \\ \bottomrule

% Results under different training iterations - caption

==> tables/additional_ablation_attr_aggre.tex <==
\begin{minipage}{0.15\textwidth}  % 0.48
\centering
\small
\def\arraystretch{1.2}  % height
\setlength\tabcolsep{0.7em}  % width
\scalebox{0.85}{  % 0.95
\begin{tabular}{ll|c}
\toprule
& Method & DZ \\ \midrule
\rowcolor{Gray}
\textbf{(I)}   & Our final method   & 34.6 \\
\textbf{(II)}  & \textbf{(I)} - WA  & 33.3 \\
\textbf{(III)} & \textbf{(I)} - NAE  & 33.3 \\
\textbf{(IV)}  & \textbf{(I)} - NCE  & 33.3 \\
\textbf{(V)}   & \textbf{(I)} - NAE \& NCE  & 33.3 \\
\bottomrule
\end{tabular}
}
% \vspace{-1.0em}
\caption{\footnotesize
\textbf{Additional Ablation - Attribute Aggregation}: We report mIoU on Dark Zurich (DZ) \cite{sakaridis2019guided} dataset.
}
\label{tbl:addi_attr_aggregation}
\end{minipage}

==> tables/attr_aggregation.tex <==
% \begin{table}[h]
% \centering
% \small
% \def\arraystretch{1.2}  % height
% \setlength\tabcolsep{0.8em}  % width
% \scalebox{0.95}{
% \begin{tabular}{ll|c}
% \toprule
% Attribute aggregation method  &  & DZ   
% \\ 
% \midrule
% Test Time Attribute Tuning  &  Attribute set 2 &  33.3 
% \\
% Post-Aggregation  &  Attribute set 2 &  34.3 
% \\  
% Pre-Aggregation (0.4:0.6)  & Attribute set 1   &  32.9 
% \\ 
% \rowcolor{Gray}
% Pre-Aggregation (0.4:0.6) & Attribute set 2    &  34.6 
% \\  
% \bottomrule
% \end{tabular}
% }
% % \vspace{-1.0em}
% \caption{
% \textbf{Results under different attribute aggregation methods}
% }
% \label{tbl:attr_aggregation}
% \vspace{-1em}
% \end{table}

==> tables/attr_generation.tex <==
% \begin{table}[h]
% \centering
% \small
% \def\arraystretch{1.2}  % height
% \setlength\tabcolsep{0.8em}  % width
% \scalebox{0.95}{
% \begin{tabular}{c|c}
% \toprule
% Attribute set   &   DZ   \\ \midrule
% Attribute set 1    &  32.9 \\
% \rowcolor{Gray}
% Attribute set 2    &  \todo{add results} \\  
% \bottomrule
% \end{tabular}
% }
% % \vspace{-1.0em}
% \caption{
% \textbf{Results under different attribute sets}:\todo{description}
% }
% \label{tbl:attr_generation}
% \vspace{-1em}
% \end{table}

==> tables/in_domain_results.tex <==
\begin{table}[h]
\centering
\small
\def\arraystretch{1.2}  % height
\setlength\tabcolsep{0.8em}  % width
\scalebox{0.95}{
\begin{tabular}{l|cc}
\toprule
   &   Pascal-VOC & ADE20K-150   \\ \midrule
CAT-Seg-B  & 93.67 &  27.51 \\ \rowcolor{Gray}
Ours-B &     93.22   & 27.19 \\  
CAT-Seg-L    & 96.62  & 31.51 \\ \rowcolor{Gray}
Ours-L     &  96.48  & 31.48\\   
CLIP-DINOiser    &  62.18 & 20.1 \\ \rowcolor{Gray}
Ours-U     &  60.82  & 20.95 \\   \bottomrule
\end{tabular}
}
% \vspace{-1.0em}
\caption{
\textbf{Zero-Shot Semantic Segmentation on In-Domain Datasets}: Our proposed \modelname maintains the performance of the baseline on in-domain datasets.
}
\label{tbl:unsupervised}
\vspace{-1em}
\end{table}

==> tables/tpt_ablations.tex <==
% \begin{table}[t]
% \centering
% \small
% \def\arraystretch{1.2}  % height
% \setlength\tabcolsep{0.8em}  % width
% \scalebox{0.95}{
% \begin{tabular}{l|c}
% \toprule
% Learnable component & DZ   \\ 
% \midrule
%  PTE       &  32.8 \\ 
%  CTE       &  32.7 \\ \rowcolor{Gray}
%  PTE + CTE &  34.6 \\ 
%   \bottomrule
% \end{tabular}
% }
% % \vspace{-1.0em}
% \caption{
% \textbf{Learnable component in TTO for the textual modality}: We ablate the impact of different learnable components (prompt token embedding (PTE), class token embedding (CTE) and both) in the gradient-based TTO module within Seg-TTO.
% }
% \label{tbl:tpt_learneable_component}
% \vspace{-1em}
% \end{table}
